Anomaly Detection for High-Dimensional Data Using Large Deviations Principle

Most current anomaly detection methods suffer from the curse of dimensionality when dealing with high-dimensional data. We propose an anomaly detection algorithm that can scale to high-dimensional data using concepts from the theory of large deviations. The proposed Large Deviations Anomaly Detection (LAD) algorithm is shown to outperform state of art anomaly detection methods on a variety of large and high-dimensional benchmark data sets. Exploiting the ability of the algorithm to scale to high-dimensional data, we propose an online anomaly detection method to identify anomalies in a collection of multivariate time series. We demonstrate the applicability of the online algorithm in identifying counties in the United States with anomalous trends in terms of COVID-19 related cases and deaths. Several of the identified anomalous counties correlate with counties with documented poor response to the COVID pandemic.

==> Results/performance_large.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/large_data/AD_dataframe_all_ranked_by_auc.png}
    \caption{Comparing LAD with existing anomaly detection algorithms using ROC-AUC on the anomaly class as the evaluation metric. For scoring based methods, instances with top $k$ scores are labeled as anomalous, where $k$ is the actual number of anomalies in the data set.}
    \label{fig:auc_large}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/large_data/AD_dataframe_all_ranked_by_comp_time_secs.png}
    \caption{Comparing computation time for anomaly detection algorithms. The values provided are in cpu seconds.}
    \label{fig:comp_time_large}
\end{figure}


==> Results/performance_ts_0.tex <==
\subsection{Anomaly Detection in Time Series Data}
This section presents the results of LAD model on COVID-19 time series data. The US county level data for deaths and confirmed cases were studied. Both total cases as well daily new cases were analyzed for anomaly detection. To bring all the counts to a baseline, the total counts in each time series were scaled to the respective county population. Missing information was replaced with zeros and counties with no population counts were eliminated from the study. 

\subsubsection{Time window vs complete history}
Two separate analyses, time series with complete trend history and data at each individual time step, were studied. From Figures \ref{fig:total_one_timestep} and \ref{fig:total_full_hist}, it can be seen that 



% To study the performance of the LAD model on real time series data, we implemented the model on COVID-19 confirmed and death trends in US counties. Total case trends were considered for analysis as compared to the new case trends to enable studying smoother curves. To bring all the counts to a baseline, the total counts in each time series were scaled to the respective county population. Missing information was replaced with zeros and counties with no population counts were eliminated from the study. 

For the analysis, the trends in deaths and confirmed cases for each county were collectively studied as a single multivariate time series. Results for death only and confirmed cases only trends across US counties are in supplementary section.

Two versions of the data were studied where the previous time steps were and were not considered. By this, we tried to distinguish the impact of the history of the time series on identifying anomalous trends. 

Considering historic trends in analysis can dilute the distinction between time series by considering the complete trend instead of the time step in question. Thus the weight associated with each time step is decreased which results in fewer but more significant anomalies. This can be seen in Figures \ref{fig:covid_ana_confirmed_1} and \ref{fig:covid_ana_deaths_1} show the anomalous time series for confirmed cases and deaths identified in when complete history has been considered at each time step and, Figures \ref{fig:covid_ana_confirmed_2} and \ref{fig:covid_ana_deaths_2} show the anomalous time series for confirmed cases and deaths identified in when each time step has been considered without the historical data.  
It can be seen that, more anomalies have been identified in the later case with higher anomaly scores. 


\subsubsection{Top anomalous US counties}
% Anomalous trends in COVID related deaths and confirmed cases identified by LAD has counties with both high death rates as well as significantly low death rates as compared to identified normal average.  
% Since anomalous trends in COVID related deaths and confirmed cases are studied, many counties with lower than baseline normal have been labelled as anomalous by LAD.
In Figures \ref{fig:covid_ana_deaths_top_high} and \ref{fig:covid_ana_deaths_top_low}, the death trends in counties with highest anomaly scores are presented. It can be seen that multiple counties in NY state have been identified as anomalous with significantly higher deaths than identified normal average. However, many counties with substantially lower deaths have also been identified by LAD. These include counties with deaths per population almost close to 0 across the entire timeline as well as counties with flattened trends as compared to increasing normal trend which can be used identify successful policies that helped achieve such results.


\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Full History}
     \label{fig:total_full_hist}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_full_history_top_10_per_capita.png}
         \caption{Total Confirmed Cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_full_history_top_10_per_capita.png}
         \caption{Total Deaths}
     \end{subfigure}
\end{figure}
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : One Time Step}
     \label{fig:total_one_timestep}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_one_timestep_top_10_per_capita.png}
         \caption{Total Confirmed Cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_one_timestep_top_10_per_capita.png}
         \caption{Total Deaths}
     \end{subfigure}
\end{figure}

\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Full History}
     \label{fig:new_full_hist}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_full_history_top_10_per_capita.png}
         \caption{New Confirmed Cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_full_history_top_10_per_capita.png}
         \caption{New Deaths}
     \end{subfigure}
\end{figure}
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : One Time Step}
     \label{fig:new_one_timestep}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_one_timestep_top_10_per_capita.png}
         \caption{New Confirmed Cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_one_timestep_top_10_per_capita.png}
         \caption{New Deaths}
     \end{subfigure}
\end{figure}

\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Full History, Uneven Time Series}
     \label{fig:total_full_hist_uneven}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_full_history_top_10_per_capita.png}
         \caption{Total Confirmed Cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_full_history_top_10_per_capita.png}
         \caption{Total Deaths}
     \end{subfigure}
\end{figure}
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : One Time Step, Uneven Time Series}
     \label{fig:total_one_timestep_uneven}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_one_timestep_top_10_per_capita.png}
         \caption{Total Confirmed Cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_one_timestep_top_10_per_capita.png}
         \caption{Total Deaths}
     \end{subfigure}
\end{figure}

\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : One Time Step, Uneven Time Series}
     \label{fig:new_one_timestep_uneven}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_new_one_timestep_top_10_per_capita.png}
         \caption{New Confirmed Cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_new_one_timestep_top_10_per_capita.png}
         \caption{New Deaths}
     \end{subfigure}
\end{figure}


\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Full History, Combined}
     \label{fig:total_full_hist_combined}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Confirmed Cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Deaths}
     \end{subfigure}
\end{figure}
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : One Time Step, Combined}
     \label{fig:total_one_timestep_combined}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Confirmed Cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Deaths}
     \end{subfigure}
\end{figure}


\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Full History, Combined}
     \label{fig:new_full_hist_combined}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_full_history_combined_top_10_per_capita.png}
         \caption{New Confirmed Cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_full_history_combined_top_10_per_capita.png}
         \caption{New Deaths}
     \end{subfigure}
\end{figure}
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : One Time Step, Combined}
     \label{fig:new_one_timestep_combined}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_one_timestep_combined_top_10_per_capita.png}
         \caption{New Confirmed Cases}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_one_timestep_combined_top_10_per_capita.png}
         \caption{New Deaths}
     \end{subfigure}
\end{figure}


\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends :  Uneven Time Series, Combined}
     \label{fig:total_full_hist_uneven_combined}
     \begin{subfigure}[b]{0.22\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Confirmed, Full History}
         \label{fig:c_total_full_hist_uneven_combined}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.22\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Deaths, Full History}
         \label{fig:d_total_full_hist_uneven_combined}
     \end{subfigure}
    %  \bigskip
    % \caption{Top 10 Counties with Anomalous Trends : Uneven Time Series, Combined}
     \label{fig:total_one_timestep_uneven_combined}
     \begin{subfigure}[b]{0.22\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Confirmed, One Time Step}
        \label{fig:c_total_one_timestep_uneven_combined}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.22\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Deaths, One Time Step}
        \label{fig:d_total_one_timestep_uneven_combined}
     \end{subfigure}
\end{figure}


In Figure \ref{fig:total_one_timestep_combined}, it is interesting to see the change in anomaly scores for Tennessee, Lake County. The score for the death trend between August and October is higher than the score at the end of the time series. This high score is associated with the high rates observed in the confirmed case trend during the same time period. As the anomaly scores for the multivariate time series, divergence in both deaths and case trends have impact over final scores at each time step. 

Figure \ref{fig:new_one_timestep} shows the top 10 counties with anomalous trends in daily new deaths and cases. This setting enables us identifying more erratic trends with sudden jumps as compared to the smoothly divergent behaviours caught by considering total deaths and cases. 
Additionally, as compared to Figure \ref{fig:total_one_timestep}, it can be seen that the anomaly score is relatively lower for Tennessee, Lake County which has been flagged anomalous by both models. This is due to the fact that most daily new cases and deaths are low in many counties which significantly brings down the relative distance between the normal average at that particular time step. Similar comparison can be seen between Figures \ref{fig:total_full_hist} and \ref{fig:new_full_hist}. 

Figures \ref{fig:total_full_hist} shows top 10 counties anomalous total case and death trends in US. 

In studying time series of uniform lengths, the top anomalous counties have had an early raise in per-capita case and deaths. This could be useful to capture early deviations in trends in many counties. 

However, this setting allows a negative bias towards counties that had had early on cases/deaths. Thus, to eliminate this bias, we consider trimming the time series for each county, where the first time step is the one with any recorded observation. This allows us to objectively compare the trends at each location. 

In Figure \ref{fig:total_full_hist_uneven}, we can see the 



In Figures \ref{fig:total_one_timestep} and \ref{fig:new_one_timestep}, 
















---------------
\subsubsection{Time window vs complete history}
Two separate analyses, time series with complete trend history and data at each individual time step, were studied. From Figures \ref{fig:total_one_timestep} and \ref{fig:total_full_hist}, it can be seen that 

% To study the performance of the LAD model on real time series data, we implemented the model on COVID-19 confirmed and death trends in US counties. Total case trends were considered for analysis as compared to the new case trends to enable studying smoother curves. To bring all the counts to a baseline, the total counts in each time series were scaled to the respective county population. Missing information was replaced with zeros and counties with no population counts were eliminated from the study. 

% For the analysis, the trends in deaths and confirmed cases for each county were collectively studied as a single multivariate time series. 
% Results for deaths and confirmed cases trends across US counties are in supplementary section.



Considering historic trends in analysis can dilute the distinction between time series by considering the complete trend instead of the time step in question. Thus the weight associated with each time step is decreased which results in fewer but more significant anomalies. This can be seen in Figures \ref{fig:covid_ana_confirmed_1} and \ref{fig:covid_ana_deaths_1} show the anomalous time series for confirmed cases and deaths identified in when complete history has been considered at each time step and, Figures \ref{fig:covid_ana_confirmed_2} and \ref{fig:covid_ana_deaths_2} show the anomalous time series for confirmed cases and deaths identified in when each time step has been considered without the historical data.  
It can be seen that, more anomalies have been identified in the later case with higher anomaly scores. 


\subsubsection{Top anomalous US counties}
% Anomalous trends in COVID related deaths and confirmed cases identified by LAD has counties with both high death rates as well as significantly low death rates as compared to identified normal average.  
% Since anomalous trends in COVID related deaths and confirmed cases are studied, many counties with lower than baseline normal have been labelled as anomalous by LAD.
In Figures \ref{fig:covid_ana_deaths_top_high} and \ref{fig:covid_ana_deaths_top_low}, the death trends in counties with highest anomaly scores are presented. It can be seen that multiple counties in NY state have been identified as anomalous with significantly higher deaths than identified normal average. However, many counties with substantially lower deaths have also been identified by LAD. These include counties with deaths per population almost close to 0 across the entire timeline as well as counties with flattened trends as compared to increasing normal trend which can be used identify successful policies that helped achieve such results.


In Figure \ref{fig:total_one_timestep_combined}, it is interesting to see the change in anomaly scores for Tennessee, Lake County. The score for the death trend between August and October is higher than the score at the end of the time series. This high score is associated with the high rates observed in the confirmed case trend during the same time period. As the anomaly scores for the multivariate time series, divergence in both deaths and case trends have impact over final scores at each time step. 

% Figure \ref{fig:new_one_timestep} shows the top 10 counties with anomalous trends in daily new deaths and cases. This setting enables us identifying more erratic trends with sudden jumps as compared to the smoothly divergent behaviours caught by considering total deaths and cases. 

% Additionally, as compared to Figure \ref{fig:total_one_timestep}, it can be seen that the anomaly score is relatively lower for Tennessee, Lake County which has been flagged anomalous by both models. This is due to the fact that most daily new cases and deaths are low in many counties which significantly brings down the relative distance between the normal average at that particular time step. Similar comparison can be seen between Figures \ref{fig:total_full_hist} and \ref{fig:new_full_hist}. 

Figures \ref{fig:total_full_hist} shows top 10 counties anomalous total case and death trends in US. 

In studying time series of uniform lengths, the top anomalous counties have had an early raise in per-capita case and deaths. This could be useful to capture early deviations in trends in many counties. 

However, this setting allows a negative bias towards counties that had had early on cases/deaths. Thus, to eliminate this bias, we consider trimming the time series for each county, where the first time step is the one with any recorded observation. This allows us to objectively compare the trends at each location. 

In Figure \ref{fig:total_full_hist_uneven}, we can see the 

In Figures \ref{fig:total_one_timestep} and \ref{fig:new_one_timestep}, 



==> Results/performance_ts_plots_0.tex <==
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends}
     \label{fig:total}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_full_history_top_10_per_capita.png}
         \caption{Total Confirmed, Full History}
     \label{fig:c_total_full_hist}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_full_history_top_10_per_capita.png}
         \caption{Total Deaths, Full History}
     \label{fig:d_total_full_hist}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_one_timestep_top_10_per_capita.png}
         \caption{Total Confirmed, One Time Step}
     \label{fig:c_total_one_timestep}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_one_timestep_top_10_per_capita.png}
         \caption{Total Deaths, One Time Step}
     \label{fig:d_total_one_timestep}
     \end{subfigure}
\end{figure}

\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends}
     \label{fig:new}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_full_history_top_10_per_capita.png}
         \caption{New Confirmed,Full History}
     \label{fig:c_new_full_hist}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_full_history_top_10_per_capita.png}
         \caption{New Deaths, Full History}
     \label{fig:d_new_full_hist}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_one_timestep_top_10_per_capita.png}
         \caption{New Confirmed, One Time Step}
     \label{fig:c_new_one_timestep}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_one_timestep_top_10_per_capita.png}
         \caption{New Deaths, One Time Step}
     \label{fig:d_new_one_timestep}
     \end{subfigure}
\end{figure}

\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Time Series of varying lengths}
     \label{fig:total_uneven}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_full_history_top_10_per_capita.png}
         \caption{Total Confirmed, Full History}
     \label{fig:c_total_full_hist_uneven}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_full_history_top_10_per_capita.png}
         \caption{Total Deaths, Full History}
     \label{fig:d_total_full_hist_uneven}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_one_timestep_top_10_per_capita.png}
         \caption{Total Confirmed, One Time Step}
     \label{fig:c_total_one_timestep_uneven}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_one_timestep_top_10_per_capita.png}
         \caption{Total Deaths, One Time Step}
     \label{fig:d_total_one_timestep_uneven}
     \end{subfigure}
\end{figure}

\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : One Time Step, Uneven Time Series}
     \label{fig:new_one_timestep_uneven}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_new_one_timestep_top_10_per_capita.png}
         \caption{New Confirmed}
         \label{fig:c_new_one_timestep_uneven}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_new_one_timestep_top_10_per_capita.png}
         \caption{New Deaths}
         \label{fig:d_new_one_timestep_uneven}
     \end{subfigure}
\end{figure}

\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Combined}
     \label{fig:total_combined}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Confirmed, Full History}
     \label{fig:c_total_full_hist_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Deaths, Full History}
     \label{fig:d_total_full_hist_combined}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Confirmed, One Time Step}
     \label{fig:c_total_one_timestep_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Deaths, One Time Step}
     \label{fig:d_total_one_timestep_combined}
     \end{subfigure}
\end{figure}

\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Combined}
     \label{fig:new_combined}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_full_history_combined_top_10_per_capita.png}
         \caption{New Confirmed, Full History}
     \label{fig:c_new_full_hist_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_full_history_combined_top_10_per_capita.png}
         \caption{New Deaths, Full History}
     \label{fig:d_new_full_hist_combined}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_one_timestep_combined_top_10_per_capita.png}
         \caption{New Confirmed, One Time Step}
     \label{fig:c_new_one_timestep_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_one_timestep_combined_top_10_per_capita.png}
         \caption{New Deaths, One Time Step}
     \label{fig:d_new_one_timestep_combined}
     \end{subfigure}
\end{figure}

\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends :  Uneven Time Series, Combined}
     \label{fig:total_uneven_combined}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Confirmed, Full History}
         \label{fig:c_total_full_hist_uneven_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Deaths, Full History}
         \label{fig:d_total_full_hist_uneven_combined}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Confirmed, One Time Step}
        \label{fig:c_total_one_timestep_uneven_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Deaths, One Time Step}
        \label{fig:d_total_one_timestep_uneven_combined}
     \end{subfigure}
\end{figure}

==> Results/performance_ts_plots_1.tex <==
% ALL TS in here

% Varying lengths, Total counts
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends: Varying lengths, Total counts}
     \label{fig:uneven_total}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_full_history_top_10_per_capita.png}
         \caption{Total Confirmed, Full History}
     \label{fig:uneven_c_total_full_hist}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_full_history_top_10_per_capita.png}
         \caption{Total Deaths, Full History}
     \label{fig:uneven_d_total_full_hist}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_one_timestep_top_10_per_capita.png}
         \caption{Total Confirmed, One Time Step}
     \label{fig:uneven_c_total_one_timestep}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_one_timestep_top_10_per_capita.png}
         \caption{Total Deaths, One Time Step}
     \label{fig:uneven_d_total_one_timestep}
     \end{subfigure}
\end{figure}

% Varying lengths, Daily New Counts
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends: Varying lengths, Daily New Counts}
     \label{fig:uneven_new}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_new_full_history_top_10_per_capita.png}
         \caption{New Confirmed,Full History}
     \label{fig:uneven_c_new_full_hist}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_new_full_history_top_10_per_capita.png}
         \caption{New Deaths, Full History}
     \label{fig:uneven_d_new_full_hist}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_new_one_timestep_top_10_per_capita.png}
         \caption{New Confirmed, One Time Step}
     \label{fig:uneven_c_new_one_timestep}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_new_one_timestep_top_10_per_capita.png}
         \caption{New Deaths, One Time Step}
     \label{fig:uneven_d_new_one_timestep}
     \end{subfigure}
\end{figure}

% Varying lengths, Total Counts, Multivariate Time Series
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Varying lengths, Total Counts, Multivariate Time Series}
     \label{fig:uneven_total_combined}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Confirmed, Full History}
     \label{fig:uneven_c_total_full_hist_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Deaths, Full History}
     \label{fig:uneven_d_total_full_hist_combined}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Confirmed, One Time Step}
     \label{fig:uneven_c_total_one_timestep_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Deaths, One Time Step}
     \label{fig:uneven_d_total_one_timestep_combined}
     \end{subfigure}
\end{figure}

% Varying lengths, Daily New Counts, Multivariate Time Series
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Varying lengths, Daily New Counts, Multivariate Time Series}
     \label{fig:uneven_new_combined}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_new_full_history_combined_top_10_per_capita.png}
         \caption{New Confirmed, Full History}
     \label{fig:uneven_c_new_full_hist_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_new_full_history_combined_top_10_per_capita.png}
         \caption{New Deaths, Full History}
     \label{fig:uneven_d_new_full_hist_combined}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_new_one_timestep_combined_top_10_per_capita.png}
         \caption{New Confirmed, One Time Step}
     \label{fig:uneven_c_new_one_timestep_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_new_one_timestep_combined_top_10_per_capita.png}
         \caption{New Deaths, One Time Step}
     \label{fig:uneven_d_new_one_timestep_combined}
     \end{subfigure}
\end{figure}


% Uniform lengths, Total counts
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends: Uniform lengths, Total counts}
     \label{fig:total}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_full_history_top_10_per_capita.png}
         \caption{Total Confirmed, Full History}
     \label{fig:c_total_full_hist}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_full_history_top_10_per_capita.png}
         \caption{Total Deaths, Full History}
     \label{fig:d_total_full_hist}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_one_timestep_top_10_per_capita.png}
         \caption{Total Confirmed, One Time Step}
     \label{fig:c_total_one_timestep}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_one_timestep_top_10_per_capita.png}
         \caption{Total Deaths, One Time Step}
     \label{fig:d_total_one_timestep}
     \end{subfigure}
\end{figure}

% Uniform lengths, Daily New Counts
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends: Uniform lengths, Daily New Counts}
     \label{fig:new}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_full_history_top_10_per_capita.png}
         \caption{New Confirmed,Full History}
     \label{fig:c_new_full_hist}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_full_history_top_10_per_capita.png}
         \caption{New Deaths, Full History}
     \label{fig:d_new_full_hist}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_one_timestep_top_10_per_capita.png}
         \caption{New Confirmed, One Time Step}
     \label{fig:c_new_one_timestep}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_one_timestep_top_10_per_capita.png}
         \caption{New Deaths, One Time Step}
     \label{fig:d_new_one_timestep}
     \end{subfigure}
\end{figure}

% Uniform lengths, Total Counts, Multivariate Time Series
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Uniform lengths, Total Counts, Multivariate Time Series}
     \label{fig:total_combined}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Confirmed, Full History}
     \label{fig:c_total_full_hist_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_full_history_combined_top_10_per_capita.png}
         \caption{Total Deaths, Full History}
     \label{fig:d_total_full_hist_combined}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Confirmed, One Time Step}
     \label{fig:c_total_one_timestep_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_total_one_timestep_combined_top_10_per_capita.png}
         \caption{Total Deaths, One Time Step}
     \label{fig:d_total_one_timestep_combined}
     \end{subfigure}
\end{figure}

% Uniform lengths, Daily New Counts, Multivariate Time Series
\begin{figure}
     \centering
     \caption{Top 10 Counties with Anomalous Trends : Uniform lengths, Daily New Counts, Multivariate Time Series}
     \label{fig:new_combined}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_full_history_combined_top_10_per_capita.png}
         \caption{New Confirmed, Full History}
     \label{fig:c_new_full_hist_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_full_history_combined_top_10_per_capita.png}
         \caption{New Deaths, Full History}
     \label{fig:d_new_full_hist_combined}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Confirmed_new_one_timestep_combined_top_10_per_capita.png}
         \caption{New Confirmed, One Time Step}
     \label{fig:c_new_one_timestep_combined}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/Deaths_new_one_timestep_combined_top_10_per_capita.png}
         \caption{New Deaths, One Time Step}
     \label{fig:d_new_one_timestep_combined}
     \end{subfigure}
\end{figure}





% %  Time Series of varying lengths, Total Counts
% \begin{figure}
%      \centering
%      \caption{Top 10 Counties with Anomalous Trends : Time Series of varying lengths, Total Counts}
%      \label{fig:total_uneven}
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_full_history_top_10_per_capita.png}
%          \caption{Total Confirmed, Full History}
%      \label{fig:c_total_full_hist_uneven}
%      \end{subfigure}
% %     \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_full_history_top_10_per_capita.png}
%          \caption{Total Deaths, Full History}
%      \label{fig:d_total_full_hist_uneven}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_one_timestep_top_10_per_capita.png}
%          \caption{Total Confirmed, One Time Step}
%      \label{fig:c_total_one_timestep_uneven}
%      \end{subfigure}
% %     \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_one_timestep_top_10_per_capita.png}
%          \caption{Total Deaths, One Time Step}
%      \label{fig:d_total_one_timestep_uneven}
%      \end{subfigure}
% \end{figure}

% % One Time Step, Uneven Time Series, New cases and new deaths
% \begin{figure}
%      \centering
%      \caption{Top 10 Counties with Anomalous Trends : One Time Step, Uneven Time Series, Daily New Counts}
%      \label{fig:new_one_timestep_uneven}
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_new_one_timestep_top_10_per_capita.png}
%          \caption{New Confirmed}
%          \label{fig:c_new_one_timestep_uneven}
%      \end{subfigure}
% %     \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_new_one_timestep_top_10_per_capita.png}
%          \caption{New Deaths}
%          \label{fig:d_new_one_timestep_uneven}
%      \end{subfigure}
% \end{figure}

% % Uneven Time Series, Multivariate Time Series, total counts only
% \begin{figure}
%      \centering
%      \caption{Top 10 Counties with Anomalous Trends :  Uneven Time Series, Multivariate Time Series}
%      \label{fig:total_uneven_combined}
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_full_history_combined_top_10_per_capita.png}
%          \caption{Total Confirmed, Full History}
%          \label{fig:c_total_full_hist_uneven_combined}
%      \end{subfigure}
% %     \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_full_history_combined_top_10_per_capita.png}
%          \caption{Total Deaths, Full History}
%          \label{fig:d_total_full_hist_uneven_combined}
%      \end{subfigure}
% \end{figure}


==> Results/ts_table.tex <==
\begin{figure*}
% Varying lengths, Total counts
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_total_full_history_top_10_per_capita.png}
         \caption{Total Confirmed, Full History}
     \label{fig:uneven_c_total_full_hist}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_total_full_history_top_10_per_capita.png}
         \caption{Total Deaths, Full History}
     \label{fig:uneven_d_total_full_hist}
     \end{subfigure}
    \vskip\baselineskip
% Varying lengths, Daily New Counts
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Confirmed_new_full_history_top_10_per_capita.png}
         \caption{New Confirmed,Full History}
     \label{fig:uneven_c_new_full_hist}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{covid_images/non-uniform/Deaths_new_full_history_top_10_per_capita.png}
         \caption{New Deaths, Full History}
     \label{fig:uneven_d_new_full_hist}
     \end{subfigure}
\end{figure*}

==> covid_cases.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
        Anderson,TX & 900 cases in July from outbreak in prison \\
        Potter TX &  Cases from amarillo prison \\
        Burleigh and Grant Forks ND & Long term care facility (spike in September), extensive testing, lack of mask mandates, sturgis motorcycle rally from south Dakota\\
        Miami-Dade Florida & Nursing homes\\
        
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


==> related_work.tex <==
\section{Related Work}
Our work closely relates to the area of anomaly detection in time series, large deviations principle based anomaly detection and high dimensional anomaly detection. In this section, we we wish to limit our review to previous approaches in LDP based anomaly detection, anomaly detection in multivariate time series and high dimensional datasets. 


\subsection{Anomaly Detection using Large Deviations Principle}


\subsection{Anomaly Detection in Time Series}

Detection of anomalous time series have been extensively explored over time\cite{gupta2013outlier}. In particular, detecting anomalous time series in a test database with respect to a reference database consisting of normal time series is widely applicable in a number of domains such as studying system health \cite{srivastava2005discovering}, medical data \cite{lin2005approximations}, astronomical data \cite{wei2006saxually,protopapas2006finding} or credit card fraud detection \cite{ferdousi2006unsupervised}. In most settings, real time detection of anomalies is needed to dispatch necessary preventive measures for damage control. This problem formulation has been broadly studied over the past few decades\cite{yankov2008disk,chan2005modeling,Chandola:2008, Chandola:2009a}. 

% Although significant progress has been made in time series anomaly detection, evolving time series is still a challenging component. Anomaly detection in time series can be broadly categorized into two groups: identifying anomalies within each time series that identify sudden anomalous events, and identifying anomalous time series that deviate from non-anomalous trend.



\subsection{Anomaly Detection in High Dimensional Data}
In particular, a large body of research exists on studying anomalies for sequential, time series and temporal datasets \cite{gupta2013outlier,aggarwal2013survey} and high dimensional data \cite{aggarwal2001outlier,angiulli2002fast}. Many anomaly detection algorithms use dimensionality reduction techniques as a pre-processing step to anomaly detection. However, many high dimensional anomalies can be detected in high dimensional problem settings and dimensionality reduction in such settings can lead to false negatives. 


% Historically, anomaly detection algorithm can be broadly classified into score based \cite{} and classification based algorithms \cite{guggilam2019integrated,chawla2013k}. 

==> results_0.tex <==
\section{Experiments}\label{experiments}
In this section, we evaluate the performance of the LAD algorithm on multi-aspect datasets. The following experiments have been conducted to study the model:
\begin{enumerate}
    \item Anomaly Detection Performance: LAD's ability to detect real-world anomalies as compared to state-of-the-art anomaly detection models is evaluated using the ground truth labels.
    \item Handling Large Data: Anomaly detection on large datasets (high observation count or high dimensionality) are studied. 
    \item Speed: The computation and execution times of different algorithms are studied and evaluated. 
    \item COVID-19 Time Series Data: We study the performance of LAD model on multiple multivariate time series datasets to identify anomalous instances within each time step as well anomalous time series amongst many.
    % \item Real-World Effectiveness
\end{enumerate}

\subsection{Datasets}
We consider a variety of publicly available benchmark data sets from different domains (See Table~\ref{tab:datadescription}) for the experimental evaluation. For the time series data, we use COVID-19 deaths and confirmed cases for US counties from John Hopkins COIVD-19 Data Repository \citep{dong2020interactive}. 
\begin{table}
  \caption{Anomaly detection benchmark data: Description of the benchmark data sets used for evaluation of the anomaly detection ({\em sources}: UCI-ML repository~\cite{Dua:2017} and Outlier Detection DataSets /ODDS~\citep{Rayana:2016}) capabilities of the proposed model. $N$ - number of instances, $d$ - number of attributes, and $a$ - fraction of known anomalies in the data set.}
  \label{tab:datadescription}
  \begin{tabular}{|l|c|c|c|}
    \toprule
    Name & $N$ & $d$ & $a$ \\
    \midrule
    Pima	         &	768	 &	8	&	34.9 \%	\\
    Mammography	     &	11183&	6	 &	2.32 \%	\\
    Breast Cancer    &	367	 &	30 &	2.72 \%	\\
    Wine	        &	129	 &	13 &	7.75 \%	\\
    Vowels	        &	1456	&	12	&	3.43 \%	\\
    Pendigits	      &	6870 &	16 &	2.27 \%	\\
    % Remove below.. KNN has better performance
    Annthyroid	     &	7200 &	6	 &	7.42 \%	\\
    Ionosphere	    &	351	&	33	&	35.9 \%	\\
    Thyroid	        &	3772	&	6	&	2.47 \%	\\
    Pen Global       &	809	 &	16 &	11.12\%\\
    Lympho	        &	148	&	18	&	4.05 \%	\\
    WBC	            &	378	&	30	&	5.56 \%	\\
    Cardio	         &	1831 &	21 &	9.61 \%	\\
    Glass	        &	214	&	9	&	4.21 \%	\\
    Breastw	        &	683	&	9	&	34.99 \%\\
    Seismic Bumps    &	2584 &	11 &	6.58 \%	\\
  \bottomrule
    % \caption{}
\end{tabular}
\end{table}

\begin{table}
  \caption{Large and High dimensional Benchmark Data}
  \label{tab:datadescription_2}
  \begin{tabular}{|l|c|c|c|}
    \toprule
    Name & $N$ & $d$ & $a$ \\
    \midrule
    HTTP	         &	567498	 &	3	&	0.4 \%	\\
    Arrhythmia	     &	452     & 274	 &	15 \%	\\
    Shuttle         &	49097	 &	9 &	7 \%	\\
    Letter          &  1600     & 32 & 6.25 \%	\\
    Musk          &  3062       & 166	&   3.2 \%	\\
    Optdigits          &  5216     & 64 & 3 \%	\\
    Speech          &  3686     & 400 & 1.65 \%	\\
    Ionosphere          &  351     & 33 & 36 \%	\\
    SMTP          &  95156     & 3 & 0.03 \%	\\
    Satimage-2          &  5803     & 36 & 1.2 \%	\\
    Forest Cover          &  286048     & 10 & 0.9 \%	\\
    KDD99          &  620098     & 29 & - \%	\\
  \bottomrule
    % \caption{}
\end{tabular}
\end{table}

\subsection{Baseline Methods and Parameter Initialization}

As described in Section \ref{methodology}, LAD falls under unsupervised learning regime targeted for high dimensional data. Here, we compare with both supervised and unsupervised offline algorithms. For this we consider Elliptic Envelope (EE)~\cite{rousseeuw1999fast}, Isolation Forest (iForest)~\cite{liu2012isolation}, {\em $k$ nearest neighbor outlier detection} (kNN)~\cite{Ramaswamy:2000}, {\em local outlier factor} (LOF)~\cite{Breunig:2000}, {\em one-class Support Vector Machines} (oc-SVM)~\cite{Tax:2004}, and {\em k-means\texttt{-{}-}}~\citep{chawla2013k}. However, KNN, (oc-SVM) and {\em k-means\texttt{-{}-}} can become computationally expensive and are not used for large datasets.
% For analysis on smaller datasets, consider four existing methods: {\em $k$ nearest neighbor outlier detection} (kNN)~\cite{Ramaswamy:2000}, {\em local outlier factor} (LOF)~\cite{Breunig:2000}, {\em one-class Support Vector Machines} (oc-SVM)~\cite{Tax:2004}, and {\em k-means\texttt{-{}-}}~\citep{chawla2013k}. 
The kNN and LOF assign an anomaly score for each data instance, while the rest of the methods provide an anomaly label. Both kNN and LOF have been previously shown to outperform other existing methods~\cite{gold2016comparative}, and are considered as the state-of-art methods. The {\em k-means\texttt{-{}-}} method performs joint clustering and anomaly detection.

 As the unsupervised methods have one or more user-defined parameters, we investigated a range of values for each parameter, and report the best results.  For the LAD model, a threshold value is required to classify observations with probability beyond the value as strictly anomalous. The initial threshold value for the experiment is set to 0.95 for benchmark datasets.
 
 All the methods for anomaly detection benchmark datasets are implemented in Python and all experiments were conducted on a 2.7 GHz Quad-Core Intel Core i7 processor with a 16 GB RAM.

\subsection{Evaluation Metrics}
As LAD is an score based algorithm, we study the ROC curves by comparing the True Positive Rate (TPR) and False Positive Rate (FPR), across various thresholds. The final ROC-AUC (Area under the ROC curve) is reported for evaluation. For time series anomaly detection, we present the final outliers and study their deviations from normal baselines.

\subsection{Anomaly Detection Performance}
The ROC-AUC measure performance of LAD and the competing algorithms is shown in Table \ref{fig:auc}. For all the listed algorithms, results for best parameter settings are reported. The proposed LAD model outperforms other methods on 2 out of 11 data sets. While other methods, especially LOF and KNN are better on other data sets, it should be noted that these methods are highly sensitive to the parameter settings. 

For larger and high-dimensional datasets, it can be seen from Tables \ref{fig:auc_large} and \ref{fig:comp_time_large} that the LAD model outperforms iForest, LOF and Elliptical Envelope in most settings. 


% The k-means−−method, which is capable of both clustering and anomaly detection, shows the best average performance. However this model requires specifying the proportion of true anomalies in the data set, which might not be feasible in a real-world setting. A specific behavior noticed in the score based INCAD model is the ranking of the anomalies. As INCAD is a conservative algorithm that identifies more anomalies, it can be seen that the model recall is relatively higher than the rest of the methods.However, the true anomalies might not always be ranked as the most anomalous observations. This behavior can be best observed in two particular datasets, namely Pen-Global and Wine data where the score based model has failed to rank most true anomaliesin the top while, the classification model still identified some of the true anomalies.
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/AD_dataframe_all_ranked_by_auc.png}
    \caption{Comparing LAD with existing anomaly detection algorithms using ROC-AUC on the anomaly class as the evaluation metric. For scoring based methods, instances with top $k$ scores are labeled as anomalous, where $k$ is the actual number of anomalies in the data set.}
    \label{fig:auc}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/AD_dataframe_all_ranked_by_comp_time_secs.png}
    \caption{Comparing computation time for anomaly detection algorithms. The values provided are in cpu seconds.}
    \label{fig:comp_time}
\end{figure}

\subsection{Anomaly Detection in Time Series Data}
To study the performance of the LAD model on real time series data, we implemented the model on COVID-19 confirmed and death trends in US counties. Total case trends were considered for analysis as compared to the new case trends to enable studying smoother curves. To bring all the counts to a baseline, the total counts in each time series were scaled to the respective county population. Missing information was replaced with zeros and counties with no population counts were eliminated from the study. 

For the analysis, the trends in deaths and confirmed cases for each county were collectively studied as a single multivariate time series. Results for death only and confirmed cases only trends across US counties are in supplementary section.

Two versions of the data were studied where the previous time steps were and were not considered. By this, we tried to distinguish the impact of the history of the time series on identifying anomalous trends. 

Considering historic trends in analysis can dilute the distinction between time series by considering the complete trend instead of the time step in question. Thus the weight associated with each time step is decreased which results in fewer but more significant anomalies. This can be seen in Figures \ref{fig:covid_ana_confirmed_1} and \ref{fig:covid_ana_deaths_1} show the anomalous time series for confirmed cases and deaths identified in when complete history has been considered at each time step and, Figures \ref{fig:covid_ana_confirmed_2} and \ref{fig:covid_ana_deaths_2} show the anomalous time series for confirmed cases and deaths identified in when each time step has been considered without the historical data.  
It can be seen that, more anomalies have been identified in the later case with higher anomaly scores. 

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/COVID/Confirmed_total_full_history_combined_ana_darker.png}
    \caption{Anomalous time series in COVID19 data for USA counties. Anomalous time series are plotted in red, where darker time series are identified to be anomalous for longer time periods. Non-anomalous time series is shown in blue. For non-anomalous behavior, the mean and the 99\% confidence interval is plotted in yellow and green respectively.}
    \label{fig:covid_ana_confirmed_1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/COVID/Deaths_total_full_history_combined_ana_darker.png}
    \caption{Anomalous time series in COVID19 data for USA counties. Anomalous time series are plotted in red, where darker time series are identified to be anomalous for longer time periods. Non-anomalous time series is shown in blue. For non-anomalous behavior, the mean and the 99\% confidence interval is plotted in yellow and green respectively.}
    \label{fig:covid_ana_deaths_1}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/COVID/Confirmed_total_one_timestep_combined_ana_darker.png}
    \caption{Anomalous time series in COVID19 data for USA counties. Anomalous time series are plotted in red, where darker time series are identified to be anomalous for longer time periods. Non-anomalous time series is shown in blue. For non-anomalous behavior, the mean and the 99\% confidence interval is plotted in yellow and green respectively.}
    \label{fig:covid_ana_confirmed_2}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/COVID/Deaths_total_one_timestep_combined_ana_darker.png}
    \caption{Anomalous time series in COVID19 data for USA counties. Anomalous time series are plotted in red, where darker time series are identified to be anomalous for longer time periods. Non-anomalous time series is shown in blue. For non-anomalous behavior, the mean and the 99\% confidence interval is plotted in yellow and green respectively.}
    \label{fig:covid_ana_deaths_2}
\end{figure}

\subsubsection{Top anomalous US counties}
% Anomalous trends in COVID related deaths and confirmed cases identified by LAD has counties with both high death rates as well as significantly low death rates as compared to identified normal average.  
% Since anomalous trends in COVID related deaths and confirmed cases are studied, many counties with lower than baseline normal have been labelled as anomalous by LAD.
In Figures \ref{fig:covid_ana_deaths_top_high} and \ref{fig:covid_ana_deaths_top_low}, the death trends in counties with highest anomaly scores are presented. It can be seen that multiple counties in NY state have been identified as anomalous with significantly higher deaths than identified normal average. However, many counties with substantially lower deaths have also been identified by LAD. These include counties with deaths per population almost close to 0 across the entire timeline as well as counties with flattened trends as compared to increasing normal trend which can be used identify successful policies that helped achieve such results.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{images/COVID/Deaths_total_full_history_combined_top10_ana_counties_low.png}
%     \caption{Top anomalous trends in COVID deaths in US counties.}
%     \label{fig:covid_ana_deaths_top_low}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{images/COVID/Confirmed_total_full_history_combined_top10_ana_counties_high.png}
%     \caption{Top anomalous trends in confirmed cases in US counties.}
%     \label{fig:covid_ana_confirmed_top_high}
% \end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/COVID/Deaths_total_full_history_top10_ana_counties_high.png}
    \caption{Top anomalous trends in COVID deaths in US counties that are above baseline average.}
    \label{fig:covid_ana_deaths_top_high}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/COVID/Deaths_total_full_history_top10_ana_counties_low.png}
    \caption{Top anomalous trends in COVID deaths in US counties that are below baseline average.}
    \label{fig:covid_ana_deaths_top_low}
\end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{images/COVID/Confirmed_total_full_history_top10_ana_counties_high.png}
%     \caption{Top anomalous trends in COVID deaths in US counties.}
%     \label{fig:covid_ana_deaths_top_low}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{images/COVID/Confirmed_total_full_history_top10_ana_counties_low.png}
%     \caption{Top anomalous trends in confirmed cases in US counties.}
%     \label{fig:covid_ana_confirmed_top_high}
% \end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/large_data/AD_dataframe_all_ranked_by_auc.png}
    \caption{Comparing LAD with existing anomaly detection algorithms using ROC-AUC on the anomaly class as the evaluation metric. For scoring based methods, instances with top $k$ scores are labeled as anomalous, where $k$ is the actual number of anomalies in the data set.}
    \label{fig:auc_large}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/large_data/AD_dataframe_all_ranked_by_comp_time_secs.png}
    \caption{Comparing computation time for anomaly detection algorithms. The values provided are in cpu seconds.}
    \label{fig:comp_time_large}
\end{figure}

